Modeling Distinct Human Interaction in Web Agents

Despite rapid progress in autonomous web agents, human involvement remains essential for shaping preferences and correcting agent behavior as tasks unfold. However, current agentic systems lack a principled understanding of when and why humans intervene, often proceeding autonomously past critical decision points or requesting unnecessary confirmation. In this work, we introduce the task of modeling human intervention to support collaborative web task execution. We collect CowCorpus, a dataset of 400 real-user web navigation trajectories containing over 4,200 interleaved human and agent actions. We identify four distinct patterns of user interaction with agents -- hands-off supervision, hands-on oversight, collaborative task-solving, and full user takeover. Leveraging these insights, we train language models (LMs) to anticipate when users are likely to intervene based on their interaction styles, yielding a 61.4-63.4% improvement in intervention prediction accuracy over base LMs. Finally, we deploy these intervention-aware models in live web navigation agents and evaluate them in a user study, finding a 36.8% increase in user-rated agent usefulness. Together, our results show structured modeling of human intervention leads to more adaptive, collaborative agents.

==> commands.tex <==
\newcommand{\lstm}{\textsc{LSTM}}
\newcommand{\ffw} {\textsc{Ffw}}
\newcommand{\attn}{\textsc{Attn}}
\newcommand{\encoder} {\textsc{Encoder}}
\newcommand{\key} {\textsc{Key}}
\newcommand{\query} {\textsc{Query}}
\newcommand{\ccca}{\textsc{Cca}}
\newcommand{\crossattention}{\textsc{Ca}}
\newcommand{\softmax}{\textrm{softmax}}
\newcommand{\ret}{\textsc{Ret}}
\newcommand{\block}{\textsc{Block}}
\newcommand{\MassiveText} {Massive Text}
\newcommand{\bert}{\textsc{Bert}\xspace}
\newcommand{\model}{\textsc{Model}}
\renewcommand{\encoder}{\textsc{Encoder}}
\newcommand{\knnlm}{k\textrm{NN-LM}}
\newcommand{\knn}{k\textrm{NN}}
\newcommand{\spalm}{\textsc{Spalm}}
\newcommand{\dpr}{\textsc{Dpr}}
\newcommand{\rag}{\textsc{RAG}}
\newcommand{\realm}{\textsc{Realm}}
\newcommand{\fid}{\textsc{FiD}}
\newcommand{\emdr}{\textsc{Emdr}^2}
\newcommand{\retro}{\textsc{Retro}\xspace}
\newcommand{\retroon}{\textsc{Retro[On]}\xspace}
\newcommand{\retrooff}{\textsc{Retro[Off]}\xspace}
\newcommand{\retrofit}{\textsc{Retro}fit\xspace}
\newcommand{\retrofitting}{\textsc{Retro}fitting\xspace}
\newcommand{\lm}{\textsc{Lm}}
\newcommand{\lmc}{\textsc{Lmc}}
\newcommand{\emb}{\textsc{Emb}}
\newcommand{\readout}{\textsc{Read}}
\newcommand{\spli}{\textsc{Split}}
\newcommand{\bpb}{\textrm{bpb}}
\newcommand{\dmodel}{d}
\newcommand{\dffw}{d_{\textrm{ffw}}}
\newcommand{\lcp}{\textrm{LCP}}

\newcommand{\datavisheader}[0]{
$C_u$ colored by loss difference & $C_u$ colored by LCP with $\ret(C_u{-1})$  & $[N_u^1, F_u^1]$ colored by LCP with $C_{u+1}$ & $[N_u^2, F_u^2]$ colored by LCP with $C_{u+1}$\\ 
$L_{\textsc{\retrooff}} - L_{\retro}\colorbox{cm_0!40}{$ \leq -0.5$}, \colorbox{cm_31!40}{$=0 $},\colorbox{cm_63!40}{$ \geq 0.5$}$
& $ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} & $ \lcp = $  \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} &
$ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} \\
\toprule}

\newcommand{\samplevisheader}[0]{
Prompt and sample of $\retrooff$  & Prompt and sample of $\retroon$ & $[N_u^1, F_u^1]$ colored by LCP with $C_{u+1}$ & $[N_u^2, F_u^2]$ colored by LCP with $C_{u+1}$\\ 

& 
colored by LCP with $\ret(C_u{-1})$ 
& & \\

&$ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} & $ \lcp = $  \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $}  &$ \lcp = $ \colorbox{cm_0!40}{$0$}, \colorbox{cm_12!40}{$1 $}, \colorbox{cm_25!40}{$2 $}, \colorbox{cm_38!40}{$3 $},\colorbox{cm_51!40}{$4 $},\colorbox{cm_63!40}{$ \geq 5 $} \\ 

\toprule}


%% Symboles avec double lignes
\newcommand{\NN}{\mathbb{N}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\SS}{\mathbb{S}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
%% Symboles arrondis
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Hh}{\mathcal{H}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Jj}{\mathcal{J}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Oo}{\mathcal{O}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Qq}{\mathcal{Q}}
\newcommand{\Rr}{\mathcal{R}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Tt}{\mathcal{T}}
\newcommand{\Uu}{\mathcal{U}}
\newcommand{\Vv}{\mathcal{V}}
\newcommand{\Ww}{\mathcal{W}}
\newcommand{\Xx}{\mathcal{X}}
\newcommand{\Yy}{\mathcal{Y}}
\newcommand{\Zz}{\mathcal{Z}}

% matrices
% \newcommand{\A}{\bm{A}}
% \newcommand{\B}{\bm{B}}
% \newcommand{\Cz}{\bm{C}}
% \newcommand{\D}{\bm{D}}
% \newcommand{\E}{\bm{E}}
% \newcommand{\F}{\bm{F}}
% \newcommand{\G}{\bm{G}}
% \newcommand{\Hz}{\bm{H}}
% \newcommand{\I}{\bm{I}}
% \newcommand{\J}{\bm{J}}
% \newcommand{\K}{\bm{K}}
% \newcommand{\Lz}{\bm{L}}
% \newcommand{\M}{\bm{M}}
% \newcommand{\N}{\bm{N}}
% \newcommand{\Oz}{\bm{O}}
% \newcommand{\Pz}{\bm{P}}
% \newcommand{\Q}{\bm{Q}}
% \newcommand{\R}{\bm{R}}
% \newcommand{\Sz}{\bm{S}}
% \newcommand{\T}{\bm{T}}
% \newcommand{\Uz}{\bm{U}}
% \newcommand{\V}{\bm{V}}
% \newcommand{\W}{\bm{W}}
% \newcommand{\X}{\bm{X}}
% \newcommand{\Y}{\bm{Y}}
% \newcommand{\Z}{\bm{Z}}

% Vectors
% \renewcommand{\a}{\bm{a}}
% \renewcommand{\b}{\bm{b}}
% \newcommand{\cz}{\bm{c}}
% \renewcommand{\d}{\bm{d}}
% \newcommand{\e}{\bm{e}}
% \newcommand{\fz}{\bm{f}}
% \newcommand{\g}{\bm{g}}
% \newcommand{\h}{\bm{h}}
% \newcommand{\iz}{\bm{i}}
% \renewcommand{\j}{\bm{j}}
% \renewcommand{\k}{\bm{k}}
% \renewcommand{\l}{\bm{l}}
% \newcommand{\m}{\bm{m}}
% \newcommand{\n}{\bm{n}}
% \renewcommand{\o}{\bm{o}}
% \newcommand{\p}{\bm{p}}
% \newcommand{\q}{\bm{q}}
% \renewcommand{\r}{\bm{r}}
% \newcommand{\s}{\bm{s}}
% \renewcommand{\t}{\bm{t}}
% \renewcommand{\uz}{\bm{u}}
% \renewcommand{\v}{\bm{v}}
% \newcommand{\w}{\bm{w}}
% \newcommand{\x}{\bm{x}}
% \newcommand{\y}{\bm{y}}
% \newcommand{\z}{\bm{z}}

% greek
\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\La}{\Lambda}
\newcommand{\si}{\sigma}
%\newcommand{\Si}{\Sigma}
\newcommand{\be}{\beta}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\renewcommand{\phi}{\varphi}
\renewcommand{\th}{\theta}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

% hat, tilde
\newcommand{\hf}{\hat f}
\newcommand{\wtf}{\tilde f}
\newcommand{\tx}{\tilde x}
\newcommand{\ta}{\tilde a}
\newcommand{\tb}{\tilde b}
\newcommand{\ty}{\tilde y}
\newcommand{\tu}{\tilde u}
\newcommand{\tv}{\tilde v}
\newcommand{\tga}{\tilde \ga}
\newcommand{\tf}{\wt{f}}



%%%%%%%%%%%%%%% MATHS OPERATORS %%%%%%%%%%%%%%%%%
\newcommand{\ins}[1]{\mathrm{#1}}
\let\Re\relax

\DeclareMathOperator{\Re}{\Rr e}
\DeclareMathOperator{\Imag}{\Ii m}
\DeclareMathOperator{\Ker}{Ker}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\Sign}{Sign}
\let\Im\relax
\DeclareMathOperator{\Im}{Im}
\DeclareMathOperator{\Corr}{Corr}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\supp}{supp}

\DeclareMathOperator{\cas}{cas}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\cotan}{cotan}
\DeclareMathOperator{\Card}{Card}
\DeclareMathOperator{\GCD}{GCD}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\interop}{int}

\newcommand{\ps}[2]{\langle #1,#2\rangle}

% regularity
\newcommand{\Calpha}{\mathrm{C}^\al}
\newcommand{\Cbeta}{\mathrm{C}^\be}
\newcommand{\Cal}{\text{C}^\al}
\newcommand{\Ctwo}{\text{C}^{2}}
\newcommand{\Calt}[1]{\text{C}^{#1}}
\newcommand{\Cder}[1]{\mathscr{C}^{#1}}
% Lp spaces
\newcommand{\lone}{\ell^1}
\newcommand{\ltwo}{\ell^2}
\newcommand{\linf}{\ell^\infty}
\newcommand{\Lone}{\text{\upshape L}^1}
\newcommand{\Ltwo}{\text{\upshape L}^2}
\newcommand{\Linf}{\text{\upshape L}^\infty}
\newcommand{\lzero}{\ell^0}
\newcommand{\lp}{\ell^p}
% circle
\newcommand{\Sun}{\text{S}^1}
% little space after forall
\newcommand{\foralls}{\forall \,}
%% for derivatives
\newcommand{\dd}{\ins{d}}
%% Use french comparaison operator
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}


%%%%%%%%%%%%%%% MATHS CONSTRUCTS %%%%%%%%%%%%%%%

%% over-symbols
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\whwh}[1]{\hat{\hat{#1}}}
\newcommand{\wt}[1]{\widetilde{#1}}
%% partial derivatives
\newcommand{\pd}[2]{ \frac{ \partial #1}{\partial #2} }
\newcommand{\pdd}[2]{ \frac{ \partial^2 #1}{\partial #2^2} }
%% nice epsilon
\renewcommand{\epsilon}{\varepsilon}
%% Pour avoir un joli i pour les complexes
\renewcommand{\imath}{\mathrm{i}}
\newcommand{\interior}[1]{\ensuremath{\overset{\circ}{#1}}}

%% Legendre symbol
\newcommand{\legsymb}[2]{ \genfrac{(}{)}{}{}{#1}{#2} }
%% exposant pour les ordinaux
\newcommand{\ordin}[2]{ ${#1}^{ \text{#2} }$ }
%% Dot product and cross product
% \newcommand{\dotp}[2]{ \left\langle #1,\,#2 \right\rangle }
\newcommand{\dotp}[2]{\langle #1,\,#2\rangle}
\newcommand{\dotps}[2]{\langle #1,\,#2\rangle}
\newcommand{\crossp}[2]{ #1 \hat #2 }
\newcommand{\seg}[2]{\llbracket #1,\,#2 \rrbracket}
\newcommand{\brac}[1]{\left[#1\right]}
%\newcommand{\norm}[1]{|\!| #1 |\!|}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\snorm}[1]{\| #1 \|}
\newcommand{\normb}[1]{\Big|\!\Big| #1 \Big |\!\Big|}
\newcommand{\normB}[1]{\left|\!\left| #1 \right|\!\right|}
\DeclareMathOperator{\diverg}{div}
\DeclareMathOperator{\Prox}{Prox}
\newcommand{\normT}[1]{\norm{#1}_{\text{T}}}
\newcommand{\normu}[1]{\norm{#1}_{1}}
\newcommand{\normi}[1]{\norm{#1}_{\infty}}
\newcommand{\normd}[1]{\norm{#1}_{2}}
\newcommand{\normz}[1]{\norm{#1}_{0}}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert} % modified by Vincent
\newcommand{\absb}[1]{\Big| #1 \Big|}

%% Function definition
\newcommand{\func}[4]{ {\left\{  \begin{array}{ccc} #1 & \longrightarrow & #2 \\ #3 & \longmapsto & #4 \end{array}  \right.} }
% transpose
% \newcommand{\transp}[1]{ {#1}^{\ins{T}} }
% l'identit�
\newcommand{\Id}{\ins{Id}}
% egal par d�finition
\newcommand{\eqdef}{\triangleq}

\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
% \DeclareMathOperator*{\sup}{sup}

%% parenthesis
\newcommand{\pa}[1]{\left( #1 \right)}
\newcommand{\bpa}[1]{\big( #1 \big)}
\newcommand{\choice}[1]{ %
	\left\{ %
		\begin{array}{l} #1 \end{array} %
	\right. }
% ensembles
\newcommand{\set}[1]{ \{ #1 \} }
\newcommand{\condset}[2]{ \left\{ #1 \;;\; #2 \right\} }


%%%%%%%%%%%%%%% SPACES %%%%%%%%%%%%%%%%%
\newcommand{\qandq}{ \quad \text{and} \quad }
\newcommand{\qqandqq}{ \qquad \text{and} \qquad }
\newcommand{\qifq}{ \quad \text{if} \quad }
\newcommand{\qqifqq}{ \qquad \text{if} \qquad }
\newcommand{\qwhereq}{ \quad \text{where} \quad }
\newcommand{\qqwhereqq}{ \qquad \text{where} \qquad }
\newcommand{\qwithq}{ \quad \text{with} \quad }
\newcommand{\qqwithqq}{ \qquad \text{with} \qquad }
\newcommand{\qforq}{ \quad \text{for} \quad }
\newcommand{\qqforqq}{ \qquad \text{for} \qquad }
\newcommand{\qqsinceqq}{ \qquad \text{since} \qquad }
\newcommand{\qsinceq}{ \quad \text{since} \quad }
\newcommand{\qarrq}{\quad\Longrightarrow\quad}
\newcommand{\qqarrqq}{\quad\Longrightarrow\quad}
\newcommand{\qiffq}{\quad\Longleftrightarrow\quad}
\newcommand{\qqiffqq}{\qquad\Longleftrightarrow\qquad}
\newcommand{\qsubjq}{ \quad \text{subject to} \quad }
\newcommand{\qqsubjqq}{ \qquad \text{subject to} \qquad }
\newcommand{\qobjq}[1]{\quad \text{#1} \quad}
\newcommand{\qqobjqq}[1]{\quad \text{#1} \quad}




% Restrictions
% Exemple: $ \rest{f}{ \Z } $

\newlength{\restsubwidth}
\newlength{\restsubheight}
\newlength{\restsubmoreheight}
\setlength{\restsubmoreheight}{4pt}
\newcommand{\rest}[2]{%
        \settowidth{\restsubwidth}{\ensuremath{#2}}
        \settoheight{\restsubheight}{\ensuremath{{}_{#2}}}
        \ensuremath{{#1\hskip 0.5pt}_{\vrule\kern2pt\parbox[b][%
        4pt][b]{\the\restsubwidth}{%
                        \ensuremath{{}_{#2}}}}}
        }

==> content.tex <==
\begin{abstract}
Despite the continuing advances in autonomous AI agents, human involvement remains essential for correcting agent behavior or disambiguate context.
However, current systems tend to either overlook user needs or interrupt users indiscriminately too frequently. 
We lack a holistic account of why users intervene, and especially of how different individuals prefer to do so.
%
In this work, we introduce the task of \textit{modeling human intervention} by predicting when humans step in during collaborative trajectories. We curate \cc{}, a dataset of human-agent collaborative web navigation sessions containing over 4.2k steps. Through analysis, we identify \zora{xxx} primary motivations for user intervention (such as error correction and preference alignment) and four representative human-agent interaction patterns, including \zora{[proactive guidance, reactive correction, iterative refinement, and shared planning]}.
%
We train language models (LMs) to (i) shift from purely autonomous to collaborative agent behavior, and (ii) adapt to distinct user intervention styles, yielding a \zora{xx.x--xx.x\%} improvement in intervention prediction accuracy.
Finally, we deploy these models in live web navigation agents. Our user study shows a xx.x\% increase in user satisfaction, demonstrating the practical value of agents that model human intervention preferences.
\end{abstract}

\input{sections/1_intro}
\input{sections/2_problem}
\input{sections/3_dataset}
\input{sections/4_modeling}
\input{sections/5_deploy-agents}
\input{sections/related-work}

\bibliography{papers}

\appendix
\input{appendix/3_dataset}
\input{appendix/4_modeling}
\input{appendix/discussions}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/impact_statement.tex <==
\section*{Impact Statement}

This paper introduces a framework for modeling human intervention in collaborative web agents, with the aim of creating agent systems that are more collaborative, reliable, and aligned with user preferences.  We analyze the impact of this research on its potential applications, ethical considerations, and societal implications. 

\textbf{Applications and Benefits}
Our work contributes to the development of safe and efficient web agents. By enabling agents to recognize their limitations and proactively seek assistance, we aim to reduce the risks associated with autonomous systems executing erroneous or irreversible actions. This paradigm ensures that agents act as helpful assistants rather than unsupervised actors.

\textbf{Data Privacy and User Agency}
Our contribution includes \cc, a dataset of real-world human interaction trajectories. We adopted following approaches to mitigate privacy risks: 
\begin{itemize}
    \item \textbf{Sensitive Data Avoidance} We explicitly instructed participants to exclude tasks that require account login or those that would expose sensitive personal metadata. 
    \item \textbf{User Control Protocol} We utilized a self-declared data collection protocol. Participants retained full agency to review their interaction logs and decide which trajectories to share and which to discard, ensuring that no accidental data leak occurred against their will. 
\end{itemize}
Due to these protocols, the resulting dataset inherently excludes sensitive information, ensuring both participant privacy and data fidelity. 

\textbf{Labor Implications}
While our focus is on assistive collaboration to augment human capabilities, we acknowledge that improvements in web agents could be applied to automate tasks currently performed by human workers. We emphasize the importance of designing agents that keep humans in the control loop to mitigate potential labor displacement. 

==> tables/PTS_step_acc_table_variation.tex <==
% PTS need to be fix
\usepackage[normalem]{ulem}
\begin{table}[]
\centering
\resizebox{0.75\columnwidth}{!}{
\begin{tabular}{lcccccccccc}
\hline
& \multirow{2}{*}{\textbf{Step Accuracy}} 
& \multicolumn{2}{c}{\textbf{F1 Score}} 
& \multirow{2}{*}{\textbf{PTS}} \\ \cline{3-4}
& & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular}
  & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} & \\ 
\hline
\multicolumn{1}{c}{\textit{Closed Source Models}} & & & & \\ \cline{1-1}

\textbf{Claude 4 Sonnet} & & & & \\
0 shot (w/o reasoning) & 0.705 & 0.245 & 0.817 & \textbf{0.302} \\
0 shot (w/ reasoning)  & 0.713 & 0.200 & 0.825 & 0.172 \\
2 shot (w/o reasoning) & \textbf{0.765} & 0.169 & \textbf{0.863} & 0.157 \\
2 shot (w/ reasoning)  & 0.733 & 0.152 & 0.842 & 0.148 \\

\textbf{GPT-4o} & & & & \\
0 shot (w/o reasoning) & 0.753 & 0.205 & 0.854 & 0.147 \\
2 shot (w/o reasoning) & 0.669 & 0.162 & 0.794 & 0.206 \\

\textbf{Gemini 2.5 Pro} & & & & \\
0 shot (w/o reasoning) & 0.697 & 0.283 & 0.808 & 0.253 \\
0 shot (w/ reasoning)  & 0.689 & 0.250 & 0.804 & 0.237 \\
2 shot (w/o reasoning) & 0.594 & 0.261 & 0.720 & 0.287 \\
2 shot (w/ reasoning)  & 0.649 & \underline{\textbf{0.313}} & 0.765 & 0.243 \\
\hline

\multicolumn{1}{c}{\textit{Open Source Models}} & & & & \\ \cline{1-1}

\textbf{Gemma 27B} & & & & \\
Base & 0.279 & 0.246 & 0.310 & 0.185 \\
Finetuned & 0.857 & 0.280 & 0.920 & \underline{\textbf{0.303}} \\

\textbf{Llava 8B} & & & & \\
Base & 0.347 & 0.000 & 0.444 & 0.001 \\
Finetuned & \underline{\textbf{0.861}} & \textbf{0.286} & \underline{\textbf{0.923}} & 0.204 \\
\hline

\multicolumn{1}{c}{\textit{Baselines}} & & & & \\ \cline{1-1}
Always Intervent & 0.139 & 0.245 & 0.000 & 0.152 \\
Always No Intervent & 0.861 & 0.000 & 0.925 & 0.000 \\
\hline

\multicolumn{5}{l}{\scriptsize \textit{Note:} All open source models are evaluated in 0-shot setting without reasoning. \textbf{Bold}: Best in group; \underline{\textbf{Underlined}}: Best overall.}
\end{tabular}
}
\caption{Step Accuracy, F1-score and PTS score for Human Intervention Prediction Task on All Data.}
\label{tab:all-data-results}
\end{table}
\begin{table}[]
\centering
\resizebox{0.75\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\hline
& \multirow{2}{*}{\textbf{Step Accuracy}} 
& \multicolumn{3}{c}{\textbf{Intervention Steps}} 
& \multirow{2}{*}{\textbf{PTS}} \\ \cline{3-5} 
& & Precision & Recall & F1 Score & \\ 
\hline
\multicolumn{1}{c}{\textit{Closed Source Models}} & & & & & \\ \cline{1-1}

\textbf{Claude 4 Sonnet} & & & & & \\
0 shot (w/o reasoning) & 0.705 & 0.190 & 0.343 & 0.245 & \textbf{0.302} \\
0 shot (w/ reasoning)  & 0.713 & 0.164 & 0.257 & 0.200 & 0.172 \\
2 shot (w/o reasoning) & \textbf{0.765} & 0.167 & 0.171 & 0.169 & 0.157 \\
2 shot (w/ reasoning)  & 0.733 & 0.136 & 0.171 & 0.152 & 0.148 \\

\textbf{GPT-4o} & & & & & \\
0 shot (w/o reasoning) & 0.753 & 0.186 & 0.229 & 0.205 & 0.147 \\
2 shot (w/o reasoning) & 0.669 & 0.125 & 0.229 & 0.162 & 0.206 \\

\textbf{Gemini 2.5 Pro} & & & & & \\
0 shot (w/o reasoning) & 0.697 & 0.211 & 0.429 & 0.283 & 0.253 \\
0 shot (w/ reasoning)  & 0.689 & 0.188 & 0.371 & 0.250 & 0.237 \\
2 shot (w/o reasoning) & 0.594 & 0.175 & 0.514 & 0.261 & 0.287 \\
2 shot (w/ reasoning)  & 0.649 & \textbf{0.215} & \textbf{0.571} & \underline{\textbf{0.313}} & 0.243 \\
\hline

\multicolumn{1}{c}{\textit{Open Source Models}} & & & & & \\ \cline{1-1}

\textbf{Gemma 27B} & & & & & \\
Base & 0.279 & 0.142 & \underline{\textbf{0.906}} & 0.246 & 0.185 \\
Finetuned & 0.857 & 0.467 & 0.200 & 0.280 & \underline{\textbf{0.303}} \\

\textbf{Llava 8B} & & & & & \\
Base & 0.347 & 0.000 & 0.000 & 0.000 & 0.001 \\
Finetuned & \underline{\textbf{0.861}} & \underline{\textbf{0.500}} & 0.200 & \textbf{0.286} & 0.204 \\
\hline

\multicolumn{1}{c}{\textit{Baselines}} & & & & & \\ \cline{1-1}
Always Intervent & 0.139 & 0.139 & 1.000 & 0.245 & 0.152 \\
Always No Intervent & 0.861 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline

\multicolumn{6}{l}{\scriptsize \textit{Note:} All open source models are evaluated in 0-shot setting without reasoning. \textbf{Bold}: Best in group; \underline{\textbf{Underlined}}: Best overall.}
\end{tabular}
}
\caption{Step Accuracy, PTS, and Intervention Steps Performance (Precision, Recall, F1) for Human Intervention Prediction Task.}
\label{tab:intervention-focused-results}
\end{table}


% all metric using original way
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccccc}
\hline
 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Step \\ Accuracy\end{tabular}}} & \multicolumn{2}{c}{\textbf{Precision}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{F1 Score}} & \multirow{2}{*}{\textbf{PTS}} \\ 
\cline{3-4} \cline{6-7} \cline{9-10}
 &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  \\ \hline

\multicolumn{1}{c}{\textit{Closed Source Models}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}

\textbf{Claude 4 Sonnet} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.716 & 0.179 & 0.884 &  & 0.324 & 0.776 &  & 0.231 & 0.826 & \textbf{0.293} \\
0 shot (w/ reasoning)  & 0.731 & 0.170 & 0.879 &  & 0.270 & 0.800 &  & 0.208 & 0.838 & 0.164 \\
2 shot (w/o reasoning) & \textbf{0.777} & 0.158 & 0.873 &  & 0.162 & \textbf{0.869} &  & 0.160 & \textbf{0.871} & 0.149 \\
2 shot (w/ reasoning)  & 0.752 & 0.149 & 0.872 &  & 0.189 & 0.837 &  & 0.167 & 0.854 & 0.158 \\

\textbf{GPT-4o} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.770 & 0.182 & 0.878 &  & 0.216 & 0.853 &  & 0.198 & 0.865 & 0.148 \\
2 shot (w/o reasoning) & 0.699 & 0.147 & 0.874 &  & 0.270 & 0.763 &  & 0.191 & 0.815 & 0.206 \\

\textbf{Gemini 2.5 Pro} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.716 & 0.213 & 0.899 &  & 0.432 & 0.759 &  & 0.286 & 0.823 & 0.262 \\
0 shot (w/ reasoning)  & 0.723 & 0.211 & 0.896 &  & 0.405 & 0.771 &  & 0.278 & 0.829 & 0.237 \\
2 shot (w/o reasoning) & 0.631 & 0.181 & 0.898 &  & 0.514 & 0.649 &  & 0.268 & 0.754 & 0.287 \\
2 shot (w/ reasoning)  & 0.681 & \textbf{0.221} & \textbf{0.914} &  & \textbf{0.568} & 0.698 &  & \textbf{0.318} & 0.792 & 0.243 \\

\hline
\multicolumn{1}{c}{\textit{SFT models}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}

\textbf{Gemma 27B (base)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.337 & 0.137 & \textbf{0.930} &  & \textbf{0.853} & 0.266 &  & 0.237 & 0.414 & 0.185 \\

\textbf{Gemma 27B (finetuned)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.869 & 0.500 & 0.891 &  & 0.216 & \textbf{0.967} &  & 0.302 & \textbf{0.928} & \textbf{0.303} \\

\textbf{Llava 8B (base)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.347 & 0.000 & 0.769 &  & 0.000 & 0.436 &  & 0.000 & 0.557 & 0.001 \\

\textbf{Llava 8B (finetuned)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.866 & \textbf{0.467} & 0.888 &  & 0.189 & 0.968 &  & \textbf{0.269} & 0.926 & 0.215 \\

\hline
\multicolumn{1}{c}{\textit{Baselines}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}

Always Intervent & 0.131 & 0.131 & 0.000 &  & 1.000 & 0.000 &  & 0.232 & 0.000 & 0.152 \\
Always No Intervent & 0.869 & 0.000 & 0.869 &  & 0.000 & 1.000 &  & 0.000 & 0.930 & 0.000 \\

\hline
\end{tabular}%
}
\caption{Step Accuracy, Precision, Recall, F1-score and PTS score for Human Intervention Prediction Task on All Data.}
\label{tab:all-data-results}
\end{table}



==> tables/clusters.tex <==
% \begin{table}[]
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{clll}
% \toprule
% \textbf{Cluster} & \textbf{\begin{tabular}[c]{@{}l@{}}Centroid values (Freq. / Intensity / \\ Mean Pos. / Hand-back Rate)\end{tabular}} & \textbf{Intervention Pattern} & \textbf{Participants} \\ \midrule
% 0 & 0.040 / 0.135 / 0.709 / 0.727 & \begin{tabular}[c]{@{}l@{}} {\color[HTML]{CB0000} {[}Mediator{]}} Rare, modest interventions, usually later in the task, \\ with a strong tendency to hand control back to the agent.\end{tabular} & \begin{tabular}[c]{@{}l@{}}P4, P5, P6, P9, P11, P12, \\ P14, P16, P17, P19, P20\end{tabular} \\ \midrule
% 1 & 0.000 / 0.000 / 0.000 / 0.000 & {\color[HTML]{32CB00} {[}Observer{]}} Never intervenes; fully hands-off throughout the task. & P1, P2, P15 \\ \midrule
% 2 & 0.116 / 0.492 / 0.764 / 0.510 & \begin{tabular}[c]{@{}l@{}} {\color[HTML]{CE6301} {[}Hands-on{]}} Frequent and substantial interventions, often later, balancing between \\ taking over and giving control back.\end{tabular} & P3, P7, P8 \\ \midrule
% 3 & 0.059 / 0.278 / 0.982 / 0.095 & \begin{tabular}[c]{@{}l@{}} {\color[HTML]{6665CD} {[}Mender{]}} Occasional interventions, but almost exclusively at the very end of the task,\\ and once they step in, they do not hand the control back to the agent.\end{tabular} & P10, P13, P18 \\ \bottomrule
% \end{tabular}%
% }
% \end{table}

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cll}
\toprule
\textbf{Cluster} & \textbf{Intervention Pattern} & \textbf{Participants} \\ \midrule
 {\color[HTML]{CB0000} Collaborative} & \begin{tabular}[c]{@{}l@{}} Rare, modest interventions, usually later in the task, \\ with a strong tendency to hand control back to the agent.\end{tabular} & \begin{tabular}[c]{@{}l@{}}P4, P5, P6, P9, P11, P12, \\ P14, P16, P17, P19, P20\end{tabular} \\ \midrule
 {\color[HTML]{32CB00} Hands-off} & Never intervenes; fully hands-off throughout the task. & P1, P2, P15 \\ \midrule
{\color[HTML]{CE6301} Hands-on}  & \begin{tabular}[c]{@{}l@{}}Frequent and substantial interventions, often later, balancing between \\ taking over and giving control back.\end{tabular} & P3, P7, P8 \\ \midrule
{\color[HTML]{6665CD} Takeover} & \begin{tabular}[c]{@{}l@{}} Occasional interventions, but almost exclusively at the very end of the task,\\ and once they step in, they do not hand the control back to the agent.\end{tabular} & P10, P13, P18 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/fixed_PTS_step_accuracy_table.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccccc}
\hline
 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Step \\ Accuracy\end{tabular}}} & \multicolumn{2}{c}{\textbf{Precision}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{F1 Score}} & \multirow{2}{*}{\textbf{PTS}} \\ \cline{3-4} \cline{6-7} \cline{9-10}
 &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  \\ \hline
\multicolumn{1}{c}{\textit{Closed Source Models}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}
\textbf{Claude 4 Sonnet} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.703 & 0.243 & 0.890 &  & 0.474 & 0.743 &  & 0.321 & 0.810 & 0.310 \\
0 shot (w/ reasoning) & 0.688 & 0.231 & 0.888 &  & 0.474 & 0.725 &  & 0.310 & 0.798 & 0.218 \\
2 shot (w/o reasoning) & 0.750 & 0.190 & 0.860 &  & 0.211 & 0.844 &  & 0.200 & 0.852 & 0.140 \\
2 shot (w/ reasoning) & 0.727 & 0.192 & 0.863 &  & 0.263 & 0.807 &  & 0.222 & 0.834 & 0.145 \\
\textbf{GPT-4o} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.758 & 0.227 & 0.868 &  & 0.263 & 0.844 &  & 0.244 & 0.856 & 0.244 \\
2 shot (w/o reasoning) & 0.727 & 0.233 & 0.878 &  & 0.368 & 0.789 &  & 0.286 & 0.831 & 0.242 \\
\textbf{Gemini 2.5 Pro} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.695 & 0.222 & 0.880 &  & 0.421 & 0.743 &  & 0.291 & 0.806 & 0.268 \\
0 shot (w/ reasoning) & 0.703 & 0.243 & 0.890 &  & 0.474 & 0.743 &  & 0.321 & 0.810 & 0.202 \\
2 shot (w/o reasoning) & 0.586 & 0.217 & 0.912 &  & 0.684 & 0.569 &  & 0.329 & 0.701 & \textbf{0.324} \\
2 shot (w/ reasoning) & 0.648 & 0.250 & \textbf{0.921} &  & 0.684 & 0.642 &  & \textbf{0.366} & 0.757 & 0.303 \\
\hline
\multicolumn{1}{c}{\textit{SFT models}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}
\textbf{Gemma 27B (base)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.291 & 0.155 & 0.875 &  & \textbf{0.842} & 0.194 &  & 0.262 & 0.318 & 0.157 \\
\textbf{Gemma 27B (finetuned)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & \textbf{0.828} & \textbf{0.333} & 0.866 &  & 0.158 & \textbf{0.945} &  & 0.214 & \textbf{0.904} & 0.298 \\
\hline
\end{tabular}%
}
\caption{Step Accuracy, Precision, Recall, F1-score and PTS score for Human Intervention Prediction Task on Fixed Tasks Only.}
\label{tab:fixed-tasks-results}
\end{table}


==> tables/free_PTS_step_accuracy_table.tex <==

\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccccccc}
\hline
 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Step \\ Accuracy\end{tabular}}} & \multicolumn{2}{c}{\textbf{Precision}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{F1 Score}} & \multirow{2}{*}{\textbf{PTS}} \\ \cline{3-4} \cline{6-7} \cline{9-10}
 &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  \\ \hline
\multicolumn{1}{c}{\textit{Closed Source Models}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}
\textbf{Claude 4 Sonnet} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.659 & 0.100 & 0.839 &  & 0.167 & 0.743 &  & 0.125 & 0.788 & 0.312 \\
0 shot (w/ reasoning) & 0.707 & 0.050 & 0.835 &  & 0.056 & 0.819 &  & 0.053 & 0.827 & 0.124 \\
2 shot (w/o reasoning) & 0.748 & 0.118 & 0.849 &  & 0.111 & 0.857 &  & 0.114 & 0.853 & 0.230 \\
2 shot (w/ reasoning) & 0.715 & 0.095 & 0.843 &  & 0.111 & 0.819 &  & 0.103 & 0.831 & 0.151 \\
\textbf{GPT-4o} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.724 & 0.136 & 0.851 &  & 0.167 & 0.819 &  & 0.150 & 0.835 & 0.045 \\
2 shot (w/o reasoning) & 0.593 & 0.079 & 0.824 &  & 0.167 & 0.667 &  & 0.107 & 0.737 & 0.187 \\
\textbf{Gemini 2.5 Pro} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.667 & 0.205 & 0.881 &  & 0.444 & 0.705 &  & 0.281 & 0.783 & 0.237 \\
0 shot (w/ reasoning) & 0.675 & 0.176 & 0.865 &  & 0.333 & 0.733 &  & 0.231 & 0.794 & 0.292 \\
2 shot (w/o reasoning) & 0.585 & 0.133 & 0.846 &  & 0.333 & 0.629 &  & 0.190 & 0.721 & 0.247 \\
2 shot (w/ reasoning) & 0.634 & 0.186 & 0.875 &  & 0.444 & 0.667 &  & 0.262 & 0.757 & 0.180 \\
\hline
\multicolumn{1}{c}{\textit{SFT models}} &  &  &  &  &  &  &  &  &  &  \\ \cline{1-1}
\textbf{Gemma 27B (base)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & 0.192 & 0.120 & 0.833 &  & \textbf{0.867} & 0.095 &  & 0.211 & 0.171 & 0.220 \\
\textbf{Gemma 27B (finetuned)} &  &  &  &  &  &  &  &  &  &  \\
0 shot (w/o reasoning) & \textbf{0.878} & \textbf{0.714} & \textbf{0.888} &  & 0.278 & \textbf{0.981} &  & \textbf{0.400} & \textbf{0.932} & \textbf{0.420} \\
\hline
\end{tabular}%
}
\caption{Step Accuracy, Precision, Recall, F1-score and PTS score for Human Intervention Prediction Task on Free-form Tasks Only.}
\label{tab:free-form-results}
\end{table}

==> tables/intervention_pred_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllllllllllllll}
\hline
 & \multicolumn{3}{c}{\textbf{Perfect Timing Score}} &  & \multicolumn{11}{c}{\textbf{Step Accuracy}} \\ \cline{2-4} \cline{6-16} 
 & \multicolumn{1}{c}{\multirow{2}{*}{Overall}} & \multicolumn{1}{c}{\multirow{2}{*}{Free-form}} & \multicolumn{1}{c}{\multirow{2}{*}{Fixed}} &  & \multicolumn{3}{c}{Overall} &  & \multicolumn{3}{c}{Free-form} &  & \multicolumn{3}{c}{Fixed} \\ \cline{6-8} \cline{10-12} \cline{14-16} 
 & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} &  & \begin{tabular}[c]{@{}l@{}}Intervention \\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Non Intervention \\ Steps\end{tabular} & All &  & \begin{tabular}[c]{@{}l@{}}Intervention \\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Non Intervention \\ Steps\end{tabular} & All &  & \begin{tabular}[c]{@{}l@{}}Intervention \\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Non Intervention \\ Steps\end{tabular} & All \\ \cline{1-8} \cline{10-12} \cline{14-16} 
\multicolumn{16}{c}{\textit{Closed sourced Models}} \\ \hline
\textbf{Claude 4 Sonnet} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
2-shot (w/ thinking) & 56.3 & 60.3 & 53.3 &  & 26.6 & 77.3 & 69.2 &  & 14 & 81.2 & 70.2 &  & 36.5 & 74.3 & 68.4 \\
2-shot (w/o thinking) & 60.1 & 65.9 & 56.2 &  & 26.7 & 81.1 & 72.7 &  & 22 & 84.7 & 74.4 &  & 30.3 & 78.7 & 71.5 \\
0-shot (w/ thinking) & 59.8 & 61.9 & 58.3 &  & 31 & 80 & 72.1 &  & 22 & 83.1 & 73.1 &  & 38.1 & 77.6 & 71.4 \\
0-shot (w/o thinking) & 61.9 & 66.2 & 59 &  & 35.7 & 79 & 72.3 &  & 32 & 83.1 & 74.8 &  & 38.5 & 76.1 & 70.6 \\
\textbf{GPT-4o} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
2-shot (w/o thinking) & 55.6 & 60 & 52.8 &  & 39.7 & 71 & 66.2 &  & 31.4 & 74.2 & 67.2 &  & 45.7 & 68.9 & 65.5 \\
0-shot (w/o thinking) & 59.6 & 60.3 & 59.2 &  & 32.8 & 81.4 & 73.9 &  & 30.8 & 84.1 & 75.3 &  & 34.3 & 79.6 & 72.9 \\
\textbf{Gemini 2.5 pro} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
2-shot (w/ thinking) & 54.8 & 58.7 & 52.2 &  & 51.7 & 59.9 & 58.6 &  & 45.1 & 65.8 & 62.4 &  & 56.5 & 56 & 56 \\
2-shot (w/o thinking) & 52.9 & 57.9 & 49.5 &  & 44.2 & 59.2 & 56.9 &  & 35.3 & 62.7 & 58.2 &  & 50.7 & 57 & 56 \\
0-shot (w/ thinking) & 55.6 & 58.9 & 53.3 &  & 30 & 77.3 & 69.9 &  & 29.4 & 76.2 & 68.5 &  & 30.4 & 78 & 70.9 \\
0-shot (w/o thinking) & 59.3 & 62.6 & 57.1 &  & 37.5 & 79.1 & 72.6 &  & 33.3 & 80.4 & 72.7 &  & 40.6 & 78.2 & 72.6 \\ \hline
\multicolumn{16}{c}{\textit{SFT models}} \\ \hline
Gemma-3-4b-it ckpt-54 & 57.3 & 68.2 & 50.8 &  & 27 & 86.7 & 76.6 &  & 31.3 & 89.4 & 78.1 &  & 23.8 & 85.2 & 75.7 \\
Gemma-3-4b-it baseline (2shot) & 33.8 & 45 & 27.1 &  & 91.9 & 17.7 & 30.3 &  & 87.5 & 19.7 & 32.9 &  & 95.2 & 16.5 & 28.7 \\
Gemma-3-4b-it baseline (zero shot) & 33.4 & 42.1 & 28.1 &  & 91.9 & 12.7 & 26.2 &  & 81.3 & 16.7 & 29.3 &  & 100 & 10.4 & 24.3 \\
Gemma-3-27b-it baseline (2shot) & 35.7 & 46.8 & 29 &  & 91.9 & 13.3 & 26.6 &  & 93.8 & 15.2 & 30.5 &  & 90.5 & 12.2 & 24.3 \\
Qwen3-32b baseline (2shot) & 33.2 & 48.5 & 23.9 &  & 54.1 & 32.6 & 36.2 &  & 56.3 & 43.9 & 46.3 &  & 52.4 & 26.1 & 30.2 \\
Qwen3-32b baseline (zero shot) & 42.8 & 53.3 & 36.4 &  & 64.9 & 52.5 & 54.6 &  & 56.3 & 56.1 & 56.1 &  & 71.4 & 50.4 & 53.7 \\
Qwen3-32b-it ckpt-90 & 61.5 & 62.8 & 60.6 &  & 21.6 & 91.2 & 79.4 &  & 6.3 & 93.9 & 76.8 &  & 33.3 & 89.6 & 80.9 \\ \cline{1-8} \cline{10-12} \cline{14-16} 
\end{tabular}%
}
\caption{\faria{work in progress. expect values to change}}
\label{tab:my-table}
\end{table}

==> tables/step_accuracy_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccccccccc}
\hline
 & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Step \\ Accuracy\end{tabular}}} & \multicolumn{2}{c}{\textbf{Precision}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{F1 Score}} \\ \cline{3-4} \cline{6-7} \cline{9-10} 
 &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} &  & \begin{tabular}[c]{@{}c@{}}Intervention\\ Steps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Non-Intervention\\ Steps\end{tabular} \\ \hline
\multicolumn{1}{c}{\textit{Closed sourced Models}} &  &  &  &  &  &  &  &  &  \\ \cline{1-1}
\textbf{Claude 4 Sonnet} &  &  &  &  &  &  &  &  &  \\
2 shot (w/ reasoning) & 0.648 & 0.147 & 0.851 &  & 0.286 & 0.711 &  & 0.194 & 0.775 \\
2 shot (w/o reasoning) & 0.636 & 0.108 & 0.836 &  & 0.2 & 0.711 &  & 0.14 & 0.769 \\
0 shot (w/ reasoning) & 0.733 & 0.231 & 0.875 &  & 0.343 & 0.801 &  & 0.276 & 0.836 \\
0 shot (w/o reasoning) & 0.729 & 0.254 & 0.887 &  & 0.429 & 0.781 &  & 0.319 & 0.831 \\
\textbf{GPT-4o} &  &  &  &  &  &  &  &  &  \\
2 shot (w/o reasoning) & 0.665 & 0.218 & 0.886 &  & 0.486 & 0.697 &  & 0.301 & 0.780 \\
0 shot (w/o reasoning) & 0.708 & 0.207 & 0.871 &  & 0.343 & 0.771 &  & 0.258 & 0.818 \\
\textbf{Gemini 2.5 pro} &  &  &  &  &  &  &  &  &  \\
2 shot (w/ reasoning) & 0.648 & 0.227 & 0.899 &  & 0.571 & 0.662 &  & 0.325 & 0.762 \\
2 shot (w/o reasoning) & 0.614 & 0.196 & 0.882 &  & 0.514 & 0.632 &  & 0.283 & 0.736 \\
0 shot (w/ reasoning) & 0.733 & 0.259 & 0.888 &  & 0.429 & 0.786 &  & 0.323 & 0.834 \\
0 shot (w/o reasoning) & \textbf{0.746} & \textbf{0.288} & 0.898 &  & 0.486 & 0.791 &  & 0.362 & 0.841 \\ \hline
\multicolumn{1}{c}{\textit{SFT models}} &  &  &  &  &  &  &  &  &  \\ \cline{1-1}
\textbf{Gemma 27b} &  &  &  &  &  &  &  &  &  \\
Baseline (2 shot) & 0.381 & 0.190 & 0.982 &  & 0.971 & 0.279 &  & 0.318 & 0.434 \\
Baseline (0 shot) & 0.360 & 0.178 & 0.946 &  & 0.914 & 0.264 &  & 0.298 & 0.412 \\
Finetuned & \textbf{0.843} & \textbf{0.462 }& 0.890 &  & 0.343 & 0.930 &  & 0.393 & 0.910 \\
\textbf{Qwen3 32b} &  &  &  &  &  &  &  &  &  \\
Baseline (2 shot) & 0.610 & 0.223 & 0.910 &  & 0.657 & 0.602 &  & 0.333 & 0.725 \\
Baseline (0 shot) & 0.445 & 0.136 & 0.837 &  & 0.514 & 0.433 &  & 0.216 & 0.570 \\
Finetuned & 0.814 & 0.304 & 0.869 &  & 0.2 & 0.920 &  & 0.241 & 0.894 \\ \hline
\end{tabular}%
}
\caption{Step Accuracy, Precision, Recall and F1-score for Human Intervention Prediction Task.}
\label{tab:my-table}
\end{table}
